Global linear stability analysis of a slit flame subject to intrinsic thermoacoustic instability

The present study makes use of the adjoint modes of the Linearized Reactive Flow (LRF) equations to investigate the Intrinsic Thermoacoustic (ITA) feedback loop of a laminar premixed slit flame. The analysis shows that the ITA feedback loop is closed by vorticity generated in the boundary layer of the slit by impinging acoustic waves penetrating the slit. In this region, adjoint vorticity shows a high sensitivity of the flow. It is also hypothesised that the ITA eigenmode smoothly transitions to a purely hydrodynamic mode -- vortex shedding -- for a passive flame. The computational domain is chosen sufficiently short so as to isolate the ITA feedback loop from cavity modes. This analysis is made possible by the holistic character of the LRF model, i.e. a direct linearization of the non-linear reactive flow equations, including explicit finite rate chemistry and avoiding idealization of the flow.

==> ICSVstyle.tex <==

% Hastily put together by
% Gergely Takacs
% 13.1.2020
% gergelytakacs@gergelytakacs.com


\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
\usepackage[letterpaper, margin=2cm]{geometry}
\usepackage{color}
\usepackage{graphicx}
\usepackage{subfigure}
\graphicspath{{graphics_fold/}}
\usepackage{epstopdf} %Converts EPS to PDF so PDFLaTeX can be used
\usepackage{times}
\usepackage{etoolbox}
\usepackage{amsmath} % assumes amsmath package installed
\usepackage{amssymb}  % assumes amsmath package installed
\usepackage{fancyhdr}
\usepackage{psfrag}
\usepackage{enumitem}
\usepackage{indentfirst}       % indent the first line of the section and subsection
\usepackage{titlesec}          % customizing the section titles
\usepackage{hyperref}
\usepackage{babel}
\usepackage{listings}
\usepackage{booktabs}

\addto\captionsenglish{\renewcommand{\refname}{REFERENCES}}

% All code, functions, variables are typed like this
\newcommand{\code}[1]{{\lstinline[columns=fixed]{#1}}} %Shorthand for code


%% Added by G. Takacs 27.1.2018 %%

\usepackage[colorinlistoftodos]{todonotes} % Cool To-Do bubbles!
%% Added by G. Takacs 27.1.2018 %%
%\todo{}

\pagestyle{fancy}			        % set default page style
\setlength{\parskip}{0pt}
\setlist{nolistsep}

% custom \thebibliography environment
\makeatletter
\renewcommand*{\@biblabel}[1]{\hfill#1.}
\makeatother

% formatting the head rule and the foot rule
\makeatletter
\patchcmd{\headrule}{\hrule}{\color{blue}\hrule}{}{}
\patchcmd{\footrule}{\hrule}{\color{blue}\hrule}{}{}
\makeatother

% set first page erase the head rule in the first page
\fancypagestyle{firstpage}{
\fancyhead{}
\fancyfoot{}
\fancyfoot[LE,RO]{\small \thepage}
\renewcommand{\headrulewidth}{0pt}
\renewcommand{\footrulewidth}{1.5pt}
}

% custom \maketitle environment
\makeatletter
\def\maketitle{
  \thispagestyle{firstpage}
\vspace*{-11mm}{\centering\includegraphics[width=0.86\textwidth]{icsv29.jpg}\\}
  {
   \vspace*{-2mm}\fontsize{11}{20}\selectfont\rmfamily{} \noindent {\bf GLOBAL LINEAR STABILITY ANALYSIS OF A SLIT FLAME SUBJECT TO INTRINSIC THERMOACOUSTIC INSTABILITY % Annual Congress of the International Institute of Acoustics and Vibration (IIAV)}
   \\

   \vspace*{-7mm}\fontsize{17}{20}\selectfont\sffamily{}  \noindent \MakeUppercase{\textbf{\@title}}

   \vspace*{3mm}\fontsize{14}{20}\selectfont\rmfamily{} \noindent \@author
  }
}
\makeatother

% setting the standard headers and footers
\fancyhead{}
\fancyfoot{}
\fancyfoot[LE]{\small ICSV29, Annual Congress of International Institute of Acoustics and Vibration (IIAV), 9-13 July 2023}
\fancyfoot[RO]{\small ICSV29, Annual Congress of International Institute of Acoustics and Vibration (IIAV), 9-13 July 2023\\
\small \thepage}
\renewcommand{\headrulewidth}{0pt}
\renewcommand{\footrulewidth}{1.5pt}

%custom section appearance
\titleformat{\section}
  {\fontsize{14}{14}\normalfont\sffamily\bfseries}
  {\thesection.}{1em}{}                % insert a point after the section number like the original .doc file

\titleformat{\subsection}
  {\normalfont\sffamily\bfseries}
  {\thesubsection}{1em}{}

\titleformat{\subsubsection}
  {\normalfont\sffamily\small}
  {\textit{\thesubsubsection}}{1em}\textit{{}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


